Revised Masses for Low Density Planets Orbiting the Disordered M-dwarf System TOI-1266

We present an analysis of 126 new radial velocity measurements from the MAROON-X spectrograph to investigate the TOI-1266 system, which hosts two transiting sub-Neptunes at 10.8 and 18.8 days. We measure masses of $M_{b}=4.01~\pm~0.55~M_{\oplus}$ for TOI-1266 b and $M_{c}=2.00~\pm~0.72~M_{\oplus}$ for TOI-1266 c. Our mass measurements agree with existing HARPS-N observations which we combined using a weighted average yielding masses for TOI-1266 b, and c of $M_{b}=4.10~\pm~0.43~M_{\oplus}$, $M_{c}=2.4~\pm~0.54~M_{\oplus}$ respectively. The combined dataset enabled a $\approx30\%$ improvement in mass precision. With bulk densities of $\rho_{b}$ = 1.25 $\pm$ 0.36 g cm$^{-3}$ and $\rho_{c}$ = 1.36 $\pm$ 0.31 g cm$^{-3}$, the planets are among the lowest density sub-Neptunes orbiting an M dwarf. They are both consistent with rocky cores surrounded by hydrogen helium envelopes. TOI-1266 c may also be consistent with a water-rich composition, but we disfavor that interpretation from an Occam's razor perspective.

==> HARPS_TOI1266_config_red_blue_d_ic_compare.tex <==
\begin{deluxetable*}{llrrrrrrr}
\tablecaption{Model Comparison}
\tablehead{\colhead{AICc Qualitative Comparison} & \colhead{Free Parameters} & \colhead{$N_{\rm free}$} & \colhead{$N_{\rm data}$} & \colhead{RMS} & \colhead{$\ln{\mathcal{L}}$} & \colhead{BIC} & \colhead{AICc} & \colhead{$\Delta$AICc}}
\startdata

  AICc Favored Model & $K_{b}$, $K_{c}$, $K_{d}$, {$\gamma$} & 13 & 271 & 2.60 & -601.30 & 1275.48 & 1230.07 & 0.00 \\

  \hline \\

  Ruled Out & $K_{b}$, $K_{d}$, {$\gamma$} & 12 & 271 & 2.71 & -617.16 & 1301.61 & 1259.59 & 29.52 \\

   & $K_{b}$, $K_{c}$, {$\gamma$} & 11 & 271 & 2.78 & -621.21 & 1304.11 & 1265.50 & 35.43 \\

   & $K_{b}$, {$\gamma$} & 10 & 271 & 2.88 & -634.27 & 1324.63 & 1289.45 & 59.38 \\

   & $K_{c}$, $K_{d}$, {$\gamma$} & 12 & 271 & 2.95 & -657.67 & 1382.64 & 1340.62 & 110.55 \\

   & $K_{c}$, {$\gamma$} & 10 & 271 & 3.06 & -672.26 & 1400.61 & 1365.43 & 135.36 \\

   & $K_{d}$, {$\gamma$} & 11 & 271 & 3.02 & -673.31 & 1408.30 & 1369.70 & 139.63 \\

   & {$\gamma$} & 9 & 271 & 3.15 & -687.38 & 1425.24 & 1393.51 & 163.44 \\

\enddata
\label{tab:comp}
\end{deluxetable*}

==> TOI1266_config_red_blue_d_ic_compare.tex <==
\begin{deluxetable*}{llrrrrrrr}
\tablecaption{Model Comparison}
\tablehead{\colhead{AICc Qualitative Comparison} & \colhead{Free Parameters} & \colhead{$N_{\rm free}$} & \colhead{$N_{\rm data}$} & \colhead{RMS} & \colhead{$\ln{\mathcal{L}}$} & \colhead{BIC} & \colhead{AICc} & \colhead{$\Delta$AICc}}
\startdata

  AICc Favored Model & $K_{b}$, $K_{c}$, $K_{d}$, {$\gamma$} & 12 & 126 & 1.72 & -242.41 & 542.91 & 511.64 & 0.00 \\

  \hline \\

  Strongly Disfavored & $K_{b}$, $K_{c}$, {$\gamma$} & 10 & 126 & 1.79 & -248.20 & 544.81 & 518.36 & 6.72 \\

   & $K_{b}$, $K_{d}$, {$\gamma$} & 11 & 126 & 1.80 & -248.12 & 549.49 & 520.61 & 8.97 \\

  \hline \\

  Ruled Out & $K_{b}$, {$\gamma$} & 9 & 126 & 1.85 & -251.94 & 547.48 & 523.50 & 11.86 \\

   & $K_{c}$, $K_{d}$, {$\gamma$} & 11 & 126 & 2.20 & -275.27 & 603.80 & 574.92 & 63.28 \\

   & $K_{c}$, {$\gamma$} & 9 & 126 & 2.21 & -278.03 & 599.64 & 575.67 & 64.03 \\

   & {$\gamma$} & 8 & 126 & 2.27 & -284.28 & 607.30 & 585.84 & 74.20 \\

   & $K_{d}$, {$\gamma$} & 10 & 126 & 2.26 & -282.51 & 613.44 & 587.00 & 75.36 \\

\enddata
\label{tab:comp}
\end{deluxetable*}
